BSDF Importance Baking: A Lightweight Neural Solution to Importance Sampling General Parametric BSDFs

Parametric Bidirectional Scattering Distribution Functions (BSDFs) are pervasively used because of their flexibility to represent a large variety of material appearances by simply tuning the parameters. While efficient evaluation of parametric BSDFs has been well-studied, high-quality importance sampling techniques for parametric BSDFs are still scarce. Existing sampling strategies either heavily rely on approximations, resulting in high variance, or solely perform sampling on a portion of the whole BSDF slice. Moreover, many of the sampling approaches are specifically paired with certain types of BSDFs. In this paper, we seek an efficient and general way for importance sampling parametric BSDFs. We notice that the nature of importance sampling is the mapping between a uniform distribution and the target distribution. Specifically, when BSDF parameters are given, the mapping that performs importance sampling on a BSDF slice can be simply recorded as a 2D image that we name as importance map. Following this observation, we accurately precompute the importance maps using a mathematical tool named optimal transport. Then we propose a lightweight neural network to efficiently compress the precomputed importance maps. In this way, we have brought parametric BSDF important sampling to the precomputation stage, avoiding heavy runtime computation. Since this process is similar to light baking where a set of images are precomputed, we name our method importance baking. Together with a BSDF evaluation network and a PDF (probability density function) query network, our method enables full multiple importance sampling (MIS) without any revision to the rendering pipeline. Our method essentially performs perfect importance sampling. Compared with previous methods, we demonstrate reduced noise levels on rendering results with a rich set of appearances.

==> paper_sampling.tex <==
\section{BSDF Importance Baking}
\label{sec:sampling}

\subsection{Understanding importance sampling}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/placeholder_720p.png}
    % \vspace{-8mm}
    \caption{An illustration of importance sampling in 2D. (Left) unit square. (Right) cos on a hemisphere?}
    \label{fig:eval_sample_gt}
    % \vspace{-3mm}
\end{figure}

Sampling is param mapping. Write equations similar to RealNVP. Use a figure from SIG03:MCRT (2D case directly). Usually from an easy-to-implement distribution, e.g. $U[0, 1]^d$ to an arbitrarily complex function.

Importance sampling is not special. It just requires that the target dist. is a normalized (constantly scaled) version of the target function.

In 1D, a typically used method is called the inversion method. Cdf. In 2D, people usually use the marginal method. We visualize the mapping acquired in 2D, where ...

In the case of our BSDF sampling, given the BSDF parameters (need definition $\epsilon$ or other symbols) and an incident direction $\omega_i$ (need to define command), importance sampling the outgoing 2D slice of the BSDF gives the mapping (the colored image mentioned above). These mapping can be precomputed and compressed. And we propose to use a lightweight neural network to learn and infer the mapping. Since this is precomputing the mapping then quickly use it during rendering, the entire process that we propose is similar to light baking in real-time rendering. Therefore, we name it importance baking.

However, it is not straightforward.

\subsection{Optimal transport for precomputed importance}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/placeholder_720p.png}
    % \vspace{-8mm}
    \caption{Potential mappings that achieve the same importance sampling is not unique. (Top row) Row column sampling result, the corresponding sampling map, binning result. (Bottom row) Optimal transport and the corresponding sampling map, binning result. Note that the row-column sampling in theory produces discontinuous mapping, thus is not suitable for NN to learn.}
    \label{fig:rc_vs_ot}
    % \vspace{-3mm}
\end{figure}


We start by analyzing the mapping acquired using the marginal method. As Fig.~\ref{} shows, .. Continuity... Therefore, we conclude that the mapping from marginal method is not suitable to for a neural network to learn.

However, one important fact that is often ignored is that, potential mappings that achieve \emph{the same importance sampling} is not unique [need citation]. Fig.~\ref{} provides a simple but convincing example, both the marginal method and XXX can .... In fact, even in 1D, there are different mapping that ... [cite triangle cut].

Therefore, we refer to another method to generate a more reliable mapping. We use optimal transport (OT). Optimal transport is a general way of finding correspondences between two or more distributions, in the sense that it minimizes ... distance, among which lies the famous EMD.

OT has been successfully introduced to computer graphics, including interpolation [cite] and sampling [cite], but seldomly used in core rendering. 

MORE
% Therefore, we briefly introduce the 



Note again, SOT is just one way of providing the mapping for the next learning step of our method. Other specific implementation of OT, such as XXX, are all available choices. We use SOT merely because it is fast enough. Given its use in the precomputation stage, we believe it does not help to prove anything to compare against different kinds of OT implementations. Moreover, from the analysis, we can also see the relationship between the RealNVP method and ours. The RealNVP, like OT or marginal methods, is yet another method that produces the mapping data, therefore is orthogonal to the lightweight importance baking scheme that we have. And as we prove later (), RealNVP is not suitable to ...


\subsection{A lightweight neural network for importance baking}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/placeholder_720p.png}
    % \vspace{-8mm}
    \caption{Illustration of our sampling network.}
    \label{fig:nn_sample}
    % \vspace{-3mm}
\end{figure}

Now that the mapping can be obtained via OT, essentially we have enough data to . As mentioned in Sec.~\ref{}, since runtime performance is crucial to rendering, the highest level design goal of the NN architecture is to keep it simple.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/placeholder_720p.png}
    % \vspace{-8mm}
    \caption{NN eval only (converged), NN sample only (converged), GT. (Use matpreivew)}
    \label{fig:eval_sample_gt}
    % \vspace{-3mm}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/placeholder_720p.png}
    % \vspace{-8mm}
    \caption{NN eval only (part contrib) + NN sample only (part contrib) = NN MIS. (Use matpreivew)}
    \label{fig:eval_sample_mis}
    % \vspace{-3mm}
\end{figure}
